LongMamba: Enhancing Mamba's Long Context Capabilities via Training-Free Receptive Field Enlargement

State space models (SSMs) have emerged as an efficient alternative to Transformer models for language modeling, offering linear computational complexity and constant memory usage as context length increases. However, despite their efficiency in handling long contexts, recent studies have shown that SSMs, such as Mamba models, generally underperform compared to Transformers in long-context understanding tasks. To address this significant shortfall and achieve both efficient and accurate long-context understanding, we propose LongMamba, a training-free technique that significantly enhances the long-context capabilities of Mamba models. LongMamba builds on our discovery that the hidden channels in Mamba can be categorized into local and global channels based on their receptive field lengths, with global channels primarily responsible for long-context capability. These global channels can become the key bottleneck as the input context lengthens. Specifically, when input lengths largely exceed the training sequence length, global channels exhibit limitations in adaptively extend their receptive fields, leading to Mamba's poor long-context performance. The key idea of LongMamba is to mitigate the hidden state memory decay in these global channels by preventing the accumulation of unimportant tokens in their memory. This is achieved by first identifying critical tokens in the global channels and then applying token filtering to accumulate only those critical tokens. Through extensive benchmarking across synthetic and real-world long-context scenarios, LongMamba sets a new standard for Mamba's long-context performance, significantly extending its operational range without requiring additional training. Our code is available at https://github.com/GATECH-EIC/LongMamba.

==> Sections/40-discussion.tex <==
\section{Limitations and Future Works}

==> Sections/text.tex <==
\section{Introduction}

The rapid advancement of Transformer-based large language models (LLMs) has demonstrated significant capabilities across a diverse array of real-world tasks, ranging from question answering~\citep{zhuang2023toolqa}, document summarization~\citep{jin2024comprehensive}, to code completion~\citep{li2022competition}. These tasks often involve processing long input sequences, such as extensive documents and sizable codebases, thus escalating the demand for LLMs to manage increasingly longer context lengths. Contemporary commercial LLMs, including Mistral Large 2~\citep{LargeEno76:online} and GPT-4~\citep{achiam2023gpt}, now feature context windows extending up to 128,000 tokens. Despite their capabilities, Transformer-based models encounter significant scalability issues as sequence lengths increase~\citep{katharopoulos2020transformers}. This is primarily due to their quadratic computational complexity and linear memory complexity, which intensify as the token-by-token decoding process allows each token to attend to all preceding tokens.

In contrast, state space models (SSMs)~\citep{gu2021combining, gu2022parameterization, gu2022efficiently} offer a recursive computation mechanism that maintains linear computational complexity and constant memory usage, which are critical for managing fixed-size hidden states efficiently. Mamba, a recent innovative SSM~\citep{gu2023mamba}, incorporates a time-variant selective update mechanism into the hidden state, achieving performance comparable to that of Transformer-based LLMs on various language modeling tasks. Despite this, Mamba models struggle with long-sequence recall compared to similarly sized Transformers, as highlighted in recent empirical studies~\citep{waleffe2024empirical, ben2024decimamba}.

To understand the aforementioned challenge, we first analyze the per-channel attention patterns~\citep{ali2024hidden} of Mamba models. We identified that the channels have distinct receptive field lengths: most channels, termed \textit{local channels}, focus on local contexts, while others, termed \textit{global channels}, have receptive fields as long as the training sequence length, enabling them to capture global information from the entire input sequence. When we extend the sequence length to an order of magnitude larger than the training sequence, we find that the receptive fields of the \textit{global channels} fail to cover the entire sequence length. This failure results from a cumulative state decay that grows exponentially with context length, rendering the \textit{global channels} unable to effectively capture global information. We hypothesize that \textbf{this failure of the \textit{global channels} to capture global information under extended sequence lengths is the root cause of Mamba's poor performance in long-context understanding}.


Inspired by the above analysis, we propose LongMamba, a training-free method that can significantly enlarge the receptive field of \textit{global channels} by selectively filtering out less important tokens. This design is motivated by our observation that the contributions of tokens to the \textit{global channels} follow an extreme power-law distribution: most tokens contribute minimally on an individual basis but collectively lead to substantial cumulative decay. By filtering these less critical tokens \celine{[do we always do so, or only when the target length is longer than the trained one?]}, LongMamba preserves the information from important tokens while mitigating the exponential hidden state decay, thereby expanding the \textit{global channels}' receptive fields to match the input sequence length. Our contributions can be summarized as follows:

\begin{itemize}

\item Through visualization and analysis, we are the first to demonstrate that hidden state channels in Mamba SSMs have distinct receptive field lengths. Based on these effective receptive field lengths, the channels can be categorized into two classes: most channels, termed \textit{local channels}, focus on local contexts, while others, termed \textit{global channels}, capture information from the entire input sequence. 

    \item We identify that the inability of global channels to capture extensive global information as context length increases, due to exponential hidden state decay with respect to context length, is a critical bottleneck in Mamba's performance on long-context tasks. This finding enhances our understanding of Mamba models and can inspire future innovations in achieving long-context capabilities for Mamba models or other SSMs.
    
    \item Building upon our findings above, we propose LongMamba, a training-free method that attempts to align the cumulative decay observed in extended sequences with the decay patterns learned during training. This adjustment significantly expands the receptive fields of global channels, enabling them to handle and process extended contexts effectively. This capability crucially improves global information capture and addresses the fundamental challenges of long-context comprehension in Mamba models.

     \item Through comprehensive benchmarking on both synthetic and real-world long-context tasks, we demonstrate that LongMamba significantly extends the operational range of pre-trained Mamba models, outperforming previous methods aimed at enhancing Mamba's context handling capabilities. \celine{For example, give a performance highlight here?}

    
\end{itemize}
